User-Guided Clustering in Heterogeneous Information Networks via Motif-Based Comprehensive Transcription

Heterogeneous information networks (HINs) with rich semantics are ubiquitous in real-world applications. For a given HIN, many reasonable clustering results with distinct semantic meaning can simultaneously exist. User-guided clustering is hence of great practical value for HINs where users provide labels to a small portion of nodes. To cater to a broad spectrum of user guidance evidenced by different expected clustering results, carefully exploiting the signals residing in the data is potentially useful. Meanwhile, as one type of complex networks, HINs often encapsulate higher-order interactions that reflect the interlocked nature among nodes and edges. Network motifs, sometimes referred to as meta-graphs, have been used as tools to capture such higher-order interactions and reveal the many different semantics. We therefore approach the problem of user-guided clustering in HINs with network motifs. In this process, we identify the utility and importance of directly modeling higher-order interactions without collapsing them to pairwise interactions. To achieve this, we comprehensively transcribe the higher-order interaction signals to a series of tensors via motifs and propose the MoCHIN model based on joint non-negative tensor factorization. This approach applies to arbitrarily many, arbitrary forms of HIN motifs. An inference algorithm with speed-up methods is also proposed to tackle the challenge that tensor size grows exponentially as the number of nodes in a motif increases. We validate the effectiveness of the proposed method on two real-world datasets and three tasks, and MoCHIN outperforms all baselines in three evaluation tasks under three different metrics. Additional experiments demonstrated the utility of motifs and the benefit of directly modeling higher-order information especially when user guidance is limited.

==> discussion.tex <==
%!TEX root = hin_motif_clus.tex

\section{Discussion}
One limitation of \mochin{} is that it may not be easily applied to very large datasets even with speed-up methods due to the complexity of the model itself.
However, \mochin would stand out in the scenario where fine-grained understanding of the network semantics is needed.
In the experiment, we have shown that \mochin can scale to HINs with tens of thousands of nodes.
We note that for user-guided clustering, it is possible the users are mostly interested in the data instances most relevant to their intention, which could be a subset of a larger dataset.
For instance, if a data mining researcher wanted to cluster DBLP authors by research group, it is possible they would not care about the nodes not relevant to data mining research.
As such the majority of the millions of nodes in DBLP can be filtered out in preprocessing, and this user-guided clustering problem would become not only manageable to \mochin but also favorable due to \mochin{}'s capability in handling fine-grained semantics.

Moreover, in the case where the network is inevitably large, one may trade the performance of \mochin for efficiency by using only relatively simple motifs.
It is also worth noting that incremental learning is possible for \mochin{} -- when new nodes are available, one do not have to retrain the model from scratch.
